Teleported free energy simulations

Escorted free energy simulations reduce dissipation with a flow field that follows the equilibrium distribution. A continuous flow, however, cannot transfer probability between metastable basins. We show that any escort then faces a variance floor set by the change in basin weights, and lift it by adding teleportation: jumps at a rate proportional to the driving rate. We derive the corresponding nonequilibrium identity, the zero-dissipation condition, and the minimal number of jumps it requires, and illustrate the gain on an exactly solvable model and a tilted double well.

==> latexmkrc <==
# Lets supplemental.tex read equation numbers from paper.aux (package xr) on Overleaf:
# whenever an external .aux is needed, compile the corresponding .tex first.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    if (!($root_filename eq $_[0])) {
        system("latexmk -cd -pdf \"$_[0]\"");
    }
}

